The bisequence of approximation coefficients for Gauss-like and Renyi-like maps on the interval

We will establish several arithmetic and geometric properties regarding the bi-sequences of approximation coefficients (BAC) associated with the two one-parameter families of piecewise-continuous Mobius transformations introduced by Haas and Molnar. The Gauss and Renyi maps, which lead to the expansions of irrational numbers on the interval as regular and backwards continued fractions, are realized as special cases. The results are natural generalizations of theorems from Diophantine approximation.

==> notationpage.tex <==

\begin{notationpage}


\begin{comment}%%%%


\vskip 15mm

\begin{enumerate}[A) ]

  \item \bf{Spaces}       
        \begin{itemize}
          \item $\ccL^2(\IR^d)$, all square integrable functions.
          \item $\ccD(\IR^d)$, all cadlag functions.
          \item $\ccC(\IR^d,\IR)$, all continuous functions from $\IR^d$ to $\IR$.
          \item $\ccC_0(\IR^d,\IR)$, those functions in $\ccC(\IR^d,\IR)$ that vanish at infinity.
          \item $\ccC_{00}(\IR^d,\IR)$, those functions in $\ccC(\IR^d,\IR)$ that have compact support.        
        \end{itemize}
        \vskip 1mm          

  \item \bf{General Operators}       
        \begin{itemize}
          \item $\cL$, $\cM$, $\hat\cL$, $\hat\cM$ : generators of a semigroup
          \item $\cP_t$, $\cQ_t$, $\hat\cP_t$, $\hat\cQ_t$ : the corresponding semigroups                    
        \end{itemize}
        \vskip 1mm          

  \item \bf{Specific Operators}   
        \begin{itemize}
          \item $Lf(x) = \nabla \cdot A(x) \nabla ~ f (x)$
          \item $\tilde Lf(x) = \nabla \cdot \tilde A(x) \nabla ~ f (x)$
          \item $L^h f(x) = \frac{1}{h^2} ~ \sum\limits_{z \in \ZZ^d} (f(x+hz)-f(x)) ~ \Cxhz$
          \item $\tilde L^h f(x) = \frac{1}{h^2} ~ \sum\limits_{z \in \ZZ^d} (f(x+hz)-f(x)) ~ \tCxhz$
          \item Semigroups: $P_t = e^{tL}$, $\tilde P_t = e^{t\tilde L}$, 
                $P_t^h = e^{tL^h}$, $\tilde P_t^h = e^{t\tilde L^h}$
        \end{itemize}
        \vskip 1mm          

  \item \bf{Markov Processes}
        \begin{itemize}
          \item $X_t^{(h)}$ is the process on $h\ZZ^d$ with generator $L^h$. 
          \item $\tilde X_t^{(h)}$ is the process on $h\ZZ^d$ with generator $\tilde L^h$. 
          \item $X_t$ is the process on $\IR^d$ with generator $L$. 
          \item $\tilde X_t$ is the process on $\IR^d$ with generator $\tilde L$. 
        \end{itemize}

  \mynewpage{1}

  \item \bf{Dirichlet Forms} \\
        In general, $\ccE_\cM(f,g) = - \langle \cM f | g \rangle$. In $\ccL^2 (\IR^d,\mu)$, the
        inner product is defined as
        \begin{equation*}
          \langle  f | g \rangle = \int\limits_{\IR^d} f(x) g(x) dx
        \end{equation*}
        while in $\ccL^2 (h\ZZ^d,\mu^h)$ it is defined as
        \begin{equation*}
          \langle  f | g \rangle = h^d ~ \sum\limits_{x \in h\ZZ^d} f(x) g(x)  .                           
        \end{equation*}
        Note the rescaling factor $h^d$. Therefore, the various Dirichlet forms are
        \begin{itemize}
          \item $\ccE(f,g) = - \displaystyle\int [\nabla \cdot A \nabla ~ f](x) ~ g(x) ~ dx$
          \item $\tilde \ccE(f,g) = - \displaystyle\int [\nabla \cdot \tilde A \nabla ~ f](x) ~ g(x) ~ dx$
          \item $\ccE^h(f,g) = \frac{1}{2} ~ h^{d-2}                 
                                  ~\sum\limits_{x,z \in \ZZ^d} (f(x+hz)-f(x))~(g(x+hz)-g(x)) ~\Cxhz$               
          \item $\tilde \ccE^{h,\varepsilon} (f,g) = \frac{1}{2} ~ h^{d-2} ~ \sum\limits_{x,z \in \ZZ^d} 
                                        (f(x+hz)-f(x)) ~ (g(x+hz)-g(x)) ~ \tCxhz$                      
        \end{itemize}
        \vskip 1mm          

  \item \bf{Our Standard Mollifier} \\
        For each $\varepsilon > 0$, we define a standard mollifier:
        \begin{equation*}
            \eta_\varepsilon (y) = \frac{1}{\varepsilon^d} \eta \left( \frac{y}{\varepsilon} \right)
        \end{equation*}
        where $\eta$ is defined as follows:
        \begin{equation*}
            \eta(y) =
            \begin{cases}
              c_d \exp \left( \frac{1}{\|y\|^2 -1} \right) & \hbox{ if } \|y\| < 1 \cr
              0                     & \hbox{ otherwise }
            \end{cases}
        \end{equation*}
        with $c_d$ chosen such that $\| \eta \|_1 = 1$.
        \vskip 1mm          

  \item \bf{Miscellaneous}   
        \begin{itemize}
          \item $c$ is a positive constant for which the actual value does not matter and
                    can change from line to line. Sometimes an index will be added for clarity.
                    
        \end{itemize}

\end{enumerate}

\end{comment}%%%

\end{notationpage}

